A study on the effect of input data length on deep learning based magnitude classifier

The rapid characterisation of earthquake parameters such as its magnitude is at the heart of Earthquake Early Warning (EEW). In traditional EEW methods the robustness in the estimation of earthquake parameters have been observed to increase with the length of input data. Since time is a crucial factor in EEW applications, in this paper we propose a deep learning based magnitude classifier and, further we investigate the effect of using five different durations of seismic waveform data after first P wave arrival of length 1s, 3s, 10s, 20s and 30s. This is accomplished by testing the performance of the proposed model that combines Convolution and Bidirectional Long-Short Term Memory units to classify waveforms based on their magnitude into three classes "noise", "low magnitude events" and "high magnitude events". Herein, any earthquake signal with magnitude equal to or above 5.0 is labelled as high magnitude. We show that the variation in the results produced by changing the length of the data, is no more than the inherent randomness in the trained models, due to their initialisation.

==> authors.tex <==
\author[fias,geo]{Megha Chakraborty} 
\author[fias,unimainz]{Darius Fenner}
\author[fias]{Wei Li} 
\author[fias,phys]{Johannes Faber} 
\author[fias, phys]{Kai Zhou}
\author[fias,geo]{Georg Rümpker}
\author[fias,phys,gsi]{Horst Stöcker} 
\author[fias]{Nishtha Srivastava} 
\ead{srivastava@fias.uni-frankfurt.de}

\affiliation[fias]{
    organization = {Frankfurt Institute for Advanced Studies},
    postcode = {60438},
    city = {Frankfurt am Main},
    country = {Germany}
}

\affiliation[geo]{
    organization = {Institute of Geosciences, Goethe-University Frankfurt},
    postcode = {60438},
    city = {Frankfurt am Main},
    country = {Germany}
}

\affiliation[phys]{
    organization = {Institute for Theoretical Physics, Goethe Universität},
    postcode = {60438},
    city = {Frankfurt am Main},
    country = {Germany}
}

\affiliation[gsi]{
    organization = {GSI Helmholtzzentrum für Schwerionenforschung GmbH},
    postcode = {64291}, 
    city = {Darmstadt},
    country = {Germany}
}

